Sequence-level Large Language Model Training with Contrastive Preference Optimization

The next token prediction loss is the dominant self-supervised training objective for large language models and has achieved promising results in a variety of downstream tasks. However, upon closer investigation of this objective, we find that it lacks an understanding of sequence-level signals, leading to a mismatch between training and inference processes. To bridge this gap, we introduce a contrastive preference optimization (CPO) procedure that can inject sequence-level information into the language model at any training stage without expensive human labeled data. Our experiments show that the proposed objective surpasses the next token prediction in terms of win rate in the instruction-following and text generation tasks.

==> latex/cpo.tex <==
\section{Our approach}
While the RL penalty with KL control \cref{eq:rlhf_objective} is widely adopted in RLHF, it can also be used directly to train LLMs: instead of a preference reward, we can use any metric that measures text qualities as the reward $r$, including ROUGE, BLEU, MAUVE, etc. The benefit of \cref{eq:rlhf_objective} over \cref{eq:mle_objective} is that $r$ guides the model over a whole sequence $\vy$, rather than just a single token. This motivates our work to investigate the possibility of using a sequence-level objective in the pretraining stage and the SFT stage of LLM.

Following \citet{rafailov2023direct}, we assume that the preference over two sequences $\vy_w$ and $\vy_l$ given $\vx$ is parameterized by the Bradley-Terry model:
\[
 P(\vy_w\succ\vy_l|\vx)=\frac{e^{r(\vx, \vy_w)}}{e^{r(\vx, \vy_l)}+e^{r(\vx, \vy_w)}}.
\]
% The optimal policy $\pi^*$ takes the aforementioned EBM form \cref{eq:rlhf_ebm}. and this EBM reprametrization 
Under the Bradley-Terry model, DPO establishes the equivalence between the original RLHF objective \cref{eq:rlhf_objective} and the following supervised objective:
%\begin{align}
%	\mathcal{L}_{\mathrm{DPO}}\left(\pi_\theta ; \pi_{\text {ref }}\right)=-\mathbb{E}_{\left(\vx, \vy_w, \vy_l\right) \sim \mathcal{D}}\left[\log \sigma\left(\beta \log \frac{\pi_\theta\left(\vy_w \mid \vx\right)}{\pi_{\text {ref }}\left(\vy_w \mid \vx\right)}-\beta \log \frac{\pi_\theta\left(\vy_l \mid \vx\right)}{\pi_{\text {ref }}\left(\vy_l \mid \vx\right)}\right)\right],
%\end{align}

\begin{align}
\begin{split}
	&\mathcal{L}_{\mathrm{DPO}}(\pi_\theta ; \pi_{\text{ref}})=\\
	&\mathbb{E}_{(\vx, \vy_w, \vy_l) \sim \mathcal{D}}\Big[ \log \sigma\Big(\beta \log \frac{\pi_\theta(\vy_w \mid \vx)}{\pi_{\text{ref}}(\vy_w \mid \vx)} \\
	&\quad -\beta \log \frac{\pi_\theta(\vy_l \mid \vx)}{\pi_{\text{ref}}(\vy_l \mid \vx)}\Big)\Big],
\end{split}
\end{align}

where $\sigma(\cdot)$ is the Sigmoid function.

We can also generalize the formulation to the Plackett-Luce model, where we have a linear ordering $\tau(\cdot)$ among $K$ sequences:

%\begin{equation}\label{eq:rankcpo}
%\begin{split}
%		&\mathcal{L}_{\mathrm{DPO}}\left(\pi_\theta, \pi_{\mathrm{ref}}\right)\\
%		&=-\mathbb{E}_{\tau, \vy_1, \ldots, \vy_K, \vx \sim \mathcal{D}}\left[\log \prod_{k=1}^K \frac{\exp \left(\beta \log \frac{\pi_\theta\left(\vy_{\tau(k)} \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_{\tau(k)} \mid \vx\right)}\right)}{\sum_{j=k}^K \exp \left(\beta \log \frac{\pi_\theta\left(\vy_{\tau(j)} \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_{\tau(j)} \mid \vx\right)}\right)}\right].
%\end{split}
%\end{equation}

\begin{equation}\label{eq:rankdpo}
\resizebox{\columnwidth}{!}{%
$
\begin{split}
		&\mathcal{L}_{\mathrm{DPO}}\left(\pi_\theta, \pi_{\mathrm{ref}}\right)=\\
		&\underset{\substack{\tau, \vx \sim \mathcal{D} \\  \vy_1, \ldots, \vy_K} }{\mathbb{E}}\left[\log \prod_{k=1}^K \frac{\exp \left(\beta \log \frac{\pi_\theta\left(\vy_{\tau(k)} \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_{\tau(k)} \mid \vx\right)}\right)}{\sum_{j=k}^K \exp \left(\beta \log \frac{\pi_\theta\left(\vy_{\tau(j)} \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_{\tau(j)} \mid \vx\right)}\right)}\right].
\end{split}
$
}
\end{equation}
Here, $\tau(1),\ldots, \tau(K)$ induce a ranking among $K$ sequences. To simplify the notation, from now on we always assume that $\vy_1\sim\mathcal{D}$ is the most preferred text appearing in the training data. 

Investigating the DPO objective, we notice two caveats for its use in the pretraining and SFT stages: 
\begin{enumerate*}[series = tobecont, itemjoin = \quad]
	\item We need human labelers to gather $\vy_w, \vy_l$.
	\item There may not be a natural ranking among negative sequences $\vy_2,\ldots\vy_K$ in terms of text quality.
\end{enumerate*}
To tackle the first point, we sample $\vy_l\sim\mathcal{A}$ where $\mathcal{A}$ is some noise distribution from which it is cheap to sample; to tackle the second point, we provide a variant objective that models a ``best-of-$K$'' event: $\vy_1$ is the best among $K$ sequences, rather than a linear ordering event $\vy_{\tau(1)}\succ \vy_{\tau(2)}\succ \ldots\succ \vy_{\tau(K)}$.
These modifications lead to our proposed CPO objective:
%\ch{I have a hard time going from the equation above to \ref{eq:rankcpo}. Is there an assumption to make here, or just a re-lableing? If it's only relabeling based on $\tau$, let's say that explicitly. Also, what is the random variable/distribution $A$? It's essential that this part is clear before the equation is built since it's one of the main contributions of the work. I suggest re-structing the formulation as follows 1/Say what you are going to do to with $A$ and $\tau$ and why then  2/Present \ref{eq:rankcpo}. Right now you make the modifications and then explain the modifications so the reader is confused.}

\begin{align}\label{eq:norankcpo}
\begin{split}
		&\mathcal{L}_{\mathrm{CPO}}\left(\pi_\theta, \pi_{\mathrm{ref}}\right)=\\
		&\underset{\substack{ (\vx,\vy_1) \sim \mathcal{D} \\  \vy_2, \ldots, \vy_K\sim\mathcal{A}} }{\mathbb{E}} \left[\log \frac{\exp \left(\beta \log \frac{\pi_\theta\left(\vy_1 \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_1 \mid \vx\right)}\right)}{\sum_{j=1}^K \exp \left(\beta \log \frac{\pi_\theta\left(\vy_j \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_j \mid \vx\right)}\right)}\right].
\end{split}
\end{align}

%\begin{equation}\label{eq:rankingnce}
%\resizebox{\columnwidth}{!}{%
%$
%\begin{split}
%		&\mathcal{L}_{\mathrm{NCE}}\left(\pi_\theta, \pi_{\mathrm{noise}}\right)=\\
%		&\underset{\substack{ (\vx,\vy_1) \sim \mathcal{D} \\  \vy_2, \ldots, \vy_K\sim \pi_{\mathrm{noise}(\vy|\vx)} } }{\mathbb{E}} \left[\log \frac{\exp \left(\beta \log \frac{\pi_\theta\left(\vy_1 \mid \vx\right)}{\pi_{\mathrm{noise}}\left(\vy_1 \mid \vx\right)}\right)}{\sum_{j=1}^K \exp \left(\beta \log \frac{\pi_\theta\left(\vy_j \mid \vx\right)}{\pi_{\mathrm{noise}}\left(\vy_j \mid \vx\right)}\right)}\right].
%\end{split}
%$
%}
%\end{equation}

If ranking information is desired, we have the following CPO objective with ranking:

\begin{equation}\label{eq:rankcpo}
\resizebox{\columnwidth}{!}{%
$
\begin{split}
		&\mathcal{L}_{\mathrm{CPO}}\left(\pi_\theta, \pi_{\mathrm{ref}}\right)=\\
	&\underset{\substack{\tau, (\vx,\vy_1) \sim \mathcal{D} \\  \vy_2, \ldots, \vy_K\sim\mathcal{A}} }{\mathbb{E}} \left[\log {\displaystyle \prod_{k=1}^K} \frac{\exp \left(\beta \log \frac{\pi_\theta\left(\vy_{\tau(k)} \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_{\tau(k)} \mid \vx\right)}\right)}{{\displaystyle \sum_{j=k}^K} \exp \left(\beta \log \frac{\pi_\theta\left(\vy_{\tau(j)} \mid \vx\right)}{\pi_{\mathrm{ref}}\left(\vy_{\tau(j)} \mid \vx\right)}\right)}\right].
\end{split}
$
}
\end{equation}


We will later discuss some possible choices of ranking signals and show that the ranking can indeed further improve the text generation quality.
%
%Unlike the similar formulation to the DPO objectives, importantly in CPO, we do not assume $\vy_1,\ldots,\vy_K\sim \mathcal{D}$, rather it can be sampled from any distribution $\mathcal{A}$. The gist of this work is how to efficiently construct $\mathcal{A}$ to improve text generation quality.

The crucial aspect of CPO is how to generate negative sequences $\vy_2,...,\vy_k \sim \mathcal{A}$. For RLHF, negative sequences are simply the ones that humans dislike. For the qualities of text generation, we implicitly model the sequence-level signal $r(\vx, \vy)$ such that $r(\vx, \vy_k)<r(\vx, \vy_1)$, $\forall k\in\{2,\ldots, K\}$. In other words, the reward $r(\cdot)$ prefers the ground truth to any other sequence. Importantly, the actual signal $r$ is not parameterized explicitly, instead it is represented by the log density ratio $\log\frac{\pi_\theta}{\pr}$. 

\subsection{Connection to noise contrastive estimation}

Noise contrastrive estimation (NCE) \citep{gutmann2010noise} is a novel estimation technique introduced to tackle the computational infeasibility of traditional likelihood-based methods in large-scale machine learning models, particularly those involving high-dimensional data. NCE diverges from typical maximum likelihood estimation by transforming the problem into a classification task, which is deeply connected to both DPO and CPO. In NCE, the model is trained to distinguish between real data and noise/synthetic data. Beyond binary classification, RankingNCE \footnote{Despite the name, it means the model is ranking the real data highest among all data, rather than learning a total ordering.} also trains the model to rank the real data higher than all noise samples \citep{ma2018noise}. 

There are two important distinctions between CPO and NCE. First, instead of training the model to distinguish between real data and noise (at which any reasonable language model should already be good), we train the model to distinguish \textit{better than a reference model does}, hence making the model better at recognizing natural text. Second, we also introduce a denser ranking signal by incorporating the similarity among embeddings of different samples. The experiments in this paper demonstrate that such a dense training signal consistently improves text generation quality.

\subsection{Synthetic negative samples}
In this work, we propose four ways to generate synthetic negative samples. The first is to autoregressively generate continuations from a reference model (trained with the next token prediction loss). We fixed the synthetic data generation strategy to be top$-k$ sampling with $k=50$. The advantage of this strategy over the forthcoming strategies is that the generated continuations are of higher quality and lead to better downstream performance, while the disadvantage is that sampling is slow. We denote these negative samples as $\textbf{autoregressive negatives (AN)}$.  One can speed up the sampling process via speculative sampling \citep{chen2023accelerating} or using a smaller or distilled model, this direction is orthogonal to our approach and can be directly incorporated into our framework. 

The second way is to directly use the continuations to other (possibly unrelated) prefixes within the same mini-batch as the negative samples. More specifically, given a batch of prefixes and continuations $\{\vx_i, \vy_i\}_{i=1}^b$, the negative samples to the prefix $\vx_i$ are composed of $\{\vy_j\}_{j\neq i}$. Although these negative samples are not difficult to distinguish, they are very simple to create and can be easily scaled up. We denote these as $\textbf{batch negatives (BN)}$.

The third way is to perform a token-level perturbation. Given a sequence $\vy = \{\vy_1,\ldots, \vy_T\}$, we randomly select $c$ percent of the positions $\{t_1,\ldots, t_j\}\subseteq [T]$, and substitute each $\vy_{t_i}$ independently based on $\pi_\theta(\vy_{t_i}|\vy_1,\ldots,\vy_{t_i})$. We call these $\textbf{meanfield negatives (MN)}$. The name is based on the fact that we use a fully separable distribution to approximate the autoregressive distribution, but note that this is not the optimal mean-field approximation. Nevertheless, computing this particular meanfield approximation does not take an additional cost, compared to estimating the best meanfield approximation. This method does not generate semantically meaningful sentences, but it does generate hard negative samples, as the model tends to give them high probabilities. 

Lastly, for each ground truth continuation, we can truncate the continuation at a random position and append an extra EOS token to the end. We denote this by $\textbf{truncation negatives (TN})$.

\subsection{Possible ranking signals}
As mentioned above, our reward implicitly prefers the ground truth over other sequences, and we do not explicitly model the reward parametrically. 
%Obviously, the suitable reward function is not unique if we were to write this function explicitly. To name a few, given a ground truth continuation $\vy_w$ and a model-generated text $\vy_l$ to a given prefix $\vx$, the empirical training data distribution $\wh P(\vy_w|\vx)>\wh P(\vy_l|\vx)$ is one such function, since the latter empirical probability is most likely $0$; since $\wh P$ is an approximation to the real language distribution $P$, likely $P$ is also a function that is consistent with the afore-mentioned implicit preference. 
The upside of implicit representation of the reward is that it bypasses the shortcuts \citep[e.g.][]{krishna2021hurdles} that are known to other explicit metrics \footnote{Note that here we are not claiming CPO does not exist any shortcuts. The statement here simply means that other existing metrics have known shortcuts.}. However, since we do not have access to a concrete score for the text quality, when presented with more than one negative sample, we do not have a direct ranking among them.

Previous work on sequence-level training \citep{liu2022brio,bengio2015scheduled} has suggested a variety of signals, including BLEU, ROGUE, and BertScore. These signals are usually specific to certain downstream tasks such as translation or summarization. In the modern era of LLMs, they have been shown to no longer align with human evaluations \citep{goyal2022news}. Since our goal is to improve text generation or instruction-following, the cosine similarity between embeddings is a more intuitive signal to measure the distance between sequences. The use of embedding for text generation quality measurement is also suggested in the MAUVE metric \citep{pillutla2021mauve}.

When presented $K$ sequences and a ranking is desired, the sequences are ranked based on their cosine similarity to the ground truth. Let $\ve_1,\ldots, \ve_K$ be the embeddings of given sequences $\vy_1,\ldots, \vy_K$ and without loss of generality assume that $\ve_1$ is the ground truth, we define $\tau(\vy_i)<\tau(\vy_j)$ if $\frac{\ip{\ve_i}{\ve_1}}{\|\ve_i\|\|\ve_1\|}>\frac{\ip{\ve_j}{\ve_1}}{\|\ve_j\|\|\ve_1\|}$, with the lower ranking index indicating the better sample. Using the objective \cref{eq:rankcpo}, this process gives us denser signals during training and can lead to better downstream performance.

Another good candidate for the ranking signal is the reward model score. In fact, since the downstream performance is judged by a reward model, this will probably yield the best test performance as well. However, one has to train and host an extra reward model, creating extra memory and computation overhead. Therefore, we did not include such a signal during training in this work.

\subsection{Approximate reverse-KL}\label{subsec:approx_reverse_kl}
In the experiment, we also show how CPO improves reverse-KL. As we discuss previously, an unavoidable issue of calculating the reverse-KL is that we do not have access to the probability of the generated sequences under the true language distribution. However, if we agree that the ability to model natural language scales with the model size, then we can approximate the true language distribution $P$ with a more capable model $\widehat P$, hence approximating the reverse-KL divergence. Since many of our tasks are conditional by nature, for example, the instruction-following task is to generate a response conditioned on the input instruction, we further consider the expected reverse-KL divergence:
\begin{align}\label{eq:reversekl}
\begin{split}
		&\E_\vx\left[\KL\p{Q(\cdot|\vx)||\widehat P(\cdot|\vx)}\right] \\
		&\approx \frac{1}{|\gX|}\sum_{\vx\in\gX}\sum_{\vy\in \gY}Q(\vy|\vx)\log\p{\frac{Q(\vy|\vx)}{\widehat P(\vy|\vx)}},
\end{split}
\end{align}
where $\gX$ is the set of inputs (e.g. instructions) in the test set, and $\gY$ is the set of generated continuations (e.g. responses).
During our evaluation, we also notice that a more capable $Q$ tends to generate sequences $\vy$ with a lower probability $Q(\vy|\vx)$, compared to a less capable $Q$. This phenomenon is indeed expected, since a more capable model should be able to generate more diverse continuations. To overcome the numerical instability with a vanishing $Q$, we also use the following surrogate: 
\begin{align}\label{eq:condprob}
\begin{split}
		&\frac{1}{|\gX|}\sum_{\vx\in\gX}\sum_{\vy\in \gY}\frac{-\log\widehat P(\vy|\vx)}{|\vy|}, \\
		&\qquad \text{where } |\vy| \text{ is the length of $\vy$.}
\end{split}
\end{align}
This is the log conditional probability normalized by length, and its usage has been justified in \citet{cho2014properties,liu2022brio,fu2023gptscore}. In particular, \citet{fu2023gptscore} has discussed the use of normalized conditional probability with the GPT evaluator.

 

==> latex/custom_command.tex <==
\usepackage{mathtools}
\usepackage{amsmath,amsfonts,amssymb,amsthm,commath}

%\usepackage[colorlinks]{hyperref} % comment out in submission!
%\usepackage{cleveref}% http://ctan.org/pkg/cleveref
\usepackage{graphicx}
\graphicspath{ {./figures/} }
\usepackage{caption}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{listings}
\usepackage{tikz,forest}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{trees}
\usetikzlibrary{er,positioning}
\usetikzlibrary{fit,positioning}
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=12.8em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
   
   
\forestset{
    .style={
        for tree={
            base=bottom,
            child anchor=north,
            align=center,
            s sep+=1cm,
    straight edge/.style={
        edge path={\noexpand\path[\forestoption{edge},thick,-{Latex}] 
        (!u.parent anchor) -- (.child anchor);}
    },
    if n children={0}
        {tier=word, draw, thick, rectangle}
        {draw, diamond, thick, aspect=2},
    if n=1{%
        edge path={\noexpand\path[\forestoption{edge},thick,-{Latex}] 
        (!u.parent anchor) -| (.child anchor) node[pos=.2, above] {Y};}
        }{
        edge path={\noexpand\path[\forestoption{edge},thick,-{Latex}] 
        (!u.parent anchor) -| (.child anchor) node[pos=.2, above] {N};}
        }
        }
    }
}
   
   
\usepackage[inline]{enumitem}

% following loops stolen from djhsu
\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname bb#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def \by{\boldsymbol y}
\def \bi{\boldsymbol i}
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\newenvironment{hproof}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}
\def\tr{\operatorname{tr}}

\def\SPAN{\textup{span}}
\def\tu{\textup{u}}
\def\P{\mathbb{P}}
\def\S{\mathbb{S}}
\def\Q{\mathbb{Q}}
\def\cF{\mathcal{F}}
\def\cP{\mathcal{P}}
\def\cI{\mathcal{I}}
\def\cH{\mathcal{H}}
\def\cO{\mathcal{O}}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\vol{\text{vol}}
\def\cost{\text{cost}}
\def\spn{\text{span}}
\def\poly{\text{poly}}
\def\pr{\pi_{\operatorname{ref}}}

\def\kl{D_{\text{KL}}}
\def\tv{D_{\text{TV}}}
%\newcommand{\todo}[1]{\textcolor{red}{#1}}
\def\enc{\text{Encode}}
\def\be{\mathbf{e}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\nf{\nabla f}
\def\veps{\varepsilon}
\newcommand*\subtxt[1]{_{\textnormal{#1}}}
\DeclareRobustCommand\_{\ifmmode\expandafter\subtxt\else\textunderscore\fi}

\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\p}[1]{\autobracket*{#1}}

\newcommand{\ip}[2]{\left\langle #1, #2 \right \rangle}
\newcommand{\mathbbm}[1]{\text{\usefont{U}{bbm}{m}{n}#1}} % from mathbbm.sty
\newcommand{\rvect}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\conv}{\text{conv}}
\newcommand{\dist}{\text{dist}}
\newcommand{\sgn}{\text{sgn}}
\newcommand{\linfty}{\ell^\infty}

\newtheorem{fact}{Fact}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{innercustomthm}{Theorem}
\newtheorem{innercustomlemma}{Lemma}
\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
%\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
\newtheorem{question}{Question}
\newtheorem{answer}{Answer}


==> latex/math_command.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> latex/prelim.tex <==
\section{Preliminary}

\paragraph{Notation} Consider a sentence of $T$ tokens $\vx=\{\vx_1,\ldots, \vx_T\}\in\gX$, and let $P$ be the unknown target language distribution, $\tilde P(\vx)$ be the empirical distribution of the training data (which is an approximation of $P$), and $Q$ be the distribution of our model at hand. Since our paper is also closely related to RLHF, we will also use $\pi$ to represent the distributions. In particular, we sometimes write $\pi_\theta$ for a distribution that is parameterized by $\theta$, where $\theta$ is usually the set of trainable parameters of the LLM; we write $\pr$ for a reference distribution that should be clear given the context. The next token prediction loss is minimizing the forward-KL between $P$ and $Q$. 

\paragraph{Forward-KL vs. reverse-KL} The forward-KL is formally defined as the following:

\begin{align*}
\begin{split}
	&\argmin_Q \KL(P||Q) \\
        & \approx \argmin_Q \KL(\tilde P||Q) \\
    & =\argmin_Q -\frac{1}{|\gX|}\sum_{\vx\in\gX}\log{Q(\vx)}.
\end{split}
\end{align*}

Since we are only optimizing $Q$, minimizing the forward-KL is equivalent to the maximum likelihood estimation (MLE) $\max \log Q$. Further decomposing $Q(\vx)=\prod_i Q(\vx_i|\vx_1^{i-1})$, we get the next token prediction loss function
\begin{align}\label{eq:mle_objective}
	\argmax_Q\sum_{\vx\in\gX} \sum_{x_t\in\vx} \log Q(\vx_t|\vx_{1}^{t-1}).
\end{align}

To actually measure the quality of the generated text, typically, we will first generate several sequences and then evaluate the quality of these generated sequences. Here we look closely at the reverse-KL:
\begin{align}
	\KL(Q||P) = \sum_{\vx\in\gX}Q(\vx)\log\p{\frac{Q(\vx)}{P(\vx)}},
\end{align}
however, since $\vx\sim Q$, and we do not have access to $P$, the reverse-KL cannot be computed exactly.

\paragraph{The equivalence of RLHF and EBM} For the completeness of this paper, we include the result of the equivalence between RLHF and EBM. For the full proofs, we refer the reader to \cite{rafailov2023direct,korbak2022rl}.

The RLHF objective is the following:
\begin{align}\label{eq:rlhf_objective}
\begin{split}
		& \max_{\pi_\theta} \E_{\vx\sim\gD, \vy\sim\pi_\theta(\vy|\vx)}[r(\vx, \vy)] \\
		& \quad-\beta \KL\p{\pi_\theta(\vy|\vx)||\pr(\vy|\vx)},
\end{split}
\end{align}
where $\vx\sim\mathcal{D}$ is a given prefix, $\vy\sim\pi_\theta(\vy|\vx)$ is a sampled continuation from the trainable model $\pi_\theta$, and $r(\vx, \vy)\in \R$ is the reward. Meanwhile, we want to control the divergence between $\pi_\theta$ and $\pr$, where $\pr$ is usually an already pretrained or finetuned LLM.
The RLHF optimum is achieved at the following EBM:
\begin{align}\label{eq:rlhf_ebm}
	\pi^*(\vy|\vx) = \frac{1}{Z(\vx)}\pr(\vy|\vx)\exp\p{\frac{1}{\beta}r(\vx,\vy)},
\end{align}
where $Z(\vx)=\sum_{\vy}\pr(\vy|\vx)\exp\p{\frac{1}{\beta}r(\vx,\vy)}$ is the partition function.




==> latex/related_work.tex <==
\section{Related work}

LLMs trained with next token prediction loss \citep{radford2019language,chung2022scaling,sanh2021multitask,zhou2023lima} have demonstrated many fascinating capabilities, including the ability to perform zero-shot or few-shot tasks \citep{radford2019language,brown2020language} and the ability to reason \citep{wei2022chain}. 

Several works have investigated the shortcomings of MLE and exposure bias. \citet{arora2022exposure} measured the accumulation of errors in language generation due to exposure bias. \citet{schmidt2019generalization} connected exposure bias to generalization. \citet{wang2020exposure} studied how exposure bias leads to hallucination in neural machine translation. To mitigate exposure bias, there exists a long line of work that has explored sequence-level training methods. \citet{bengio2015scheduled,ranzato2015sequence} proposed to train RNN with RL or RL-related algorithms rather than teacher-forcing. BRIO \citet{liu2022brio} targeted the summarization task with the ROUGE signal. \citet{pang2020text} trained the language models with an offline RL learning algorithm. 

Recently, RLHF \citep{stiennon2020learning,ouyang2022training} was developed. Although the primary goal of RLHF is model alignment, it is effectively a sequence-level training technique. For the RLHF training, we usually need to gather a pair of continuations for each prefix, where one continuation aligns with human preference and the other does not. This pair of sequences is used to train a reward model, which is later used to supervise the samples generated by the RL-trained model. The model is typically optimized by REINFORCE \citep{williams1992simple} or PPO \citep{schulman2017proximal}. 

Sequence-level training is also closely related to energy-based models (EBM) \citep{korbak2022rl}, for example, the RLHF objective can be reframed as a supervised learning algorithm coined as direct preference optimization (DPO) \citep{rafailov2023direct} under the assumption of the Bradley-Terry model \citep{bradley1952rank} or the Plackett-Luce model \citep{plackett1975analysis,luce2012individual}. The particular formulation of the EBM in DPO mimics the formulation in \citet{deng2020residual}, with the reward function being the energy function. However, \citet{deng2020residual} directly treat the EBM as a language model, which is computationally heavy for sampling and inference (due to the estimation of the partition function). This EBM form has also been studied in controlled text generation. \citet{kumar2022gradient} adopted the Langevin dynamics technique to directly sample from the EBM, with different energy functions that characterize toxicity, fluency, and diversity. All of these methods can be viewed as sequence-level algorithms for different purposes. 

==> prelim.tex <==
\section{Preliminary}

\paragraph{Notation} Consider a sentence of $T$ tokens $\vx=\{\vx_1,\ldots, \vx_T\}\in\gX$, and let $P$ be the unknown target language distribution, $\tilde P(\vx)$ be the empirical distribution of the training data (which is an approximation of $P$), and $Q$ be the distribution of our model at hand. Since our paper is also closely related to RLHF, we will also use $\pi$ to represent the distributions. In particular, we sometimes write $\pi_\theta$ for a distribution that is parameterized by $\theta$, where $\theta$ is usually the set of trainable parameters of the LLM; we write $\pr$ for a reference distribution that should be clear given the context. The next token prediction loss is minimizing the forward-KL between $P$ and $Q$. 




